ReGraph: Scaling Graph Processing on HBM-enabled FPGAs with Heterogeneous Pipelines

The use of FPGAs for efficient graph processing has attracted significant interest. Recent memory subsystem upgrades including the introduction of HBM in FPGAs promise to further alleviate memory bottlenecks. However, modern multi-channel HBM requires much more processing pipelines to fully utilize its bandwidth potential. Existing designs do not scale well, resulting in underutilization of the HBM facilities even when all other resources are fully consumed. In this paper, we re-examined the graph processing workloads and found much diversity in processing. We also found that the diverse workloads can be easily classified into two types, namely dense and sparse partitions. This motivates us to propose a resource-efficient heterogeneous pipeline architecture. Our heterogeneous architecture comprises of two types of pipelines: Little pipelines to process dense partitions with good locality and Big pipelines to process sparse partitions with the extremely poor locality. Unlike traditional monolithic pipeline designs, the heterogeneous pipelines are tailored for more specific memory access patterns, and hence are more lightweight, allowing the architecture to scale up to more effectively with limited resources. In addition, we propose a model-guided task scheduling method that schedules partitions to the right pipeline types, generates the most efficient pipeline combination and balances workloads. Furthermore, we develop an automated open-source framework, called ReGraph, which automates the entire development process. ReGraph outperforms state-of-the-art FPGA accelerators by up to 5.9 times in terms of performance and 12times in terms of resource efficiency.

==> 1-introduction-yC.tex <==
\section{Introduction}\label{sec:introduction}
Graphs are de facto data structures to represent the relationships between entities in many application domains such as social networks, genomics, and machine learning~\cite{GraphLab, Graph500}. 
As a result, efficient graph processing is becoming increasingly important, especially as the amount of graph data grows.
Allowing efficient customization on the hardware logic to computation/memory access patterns, FPGA usually delivers better memory efficiency and energy efficiency than CPUs/GPUs~\cite{Zhou2018CF,Zhou2016,ForeGraph,graphgen,zhou2019hitgraph,chen2019fly,chen2021thundergp,isca2021,ruoshi2019improving}.
Furthermore, high-level synthesis (HLS) translates kernels written in high-level languages to low-level RTL modules alleviates the poor programmability issue of FPGAs, providing high usability to efficient graph processing systems~\cite{guo2021autobridge,HLSsurvey2016,chen2021thundergp}.


While graph processing is data access-intensive, recent High Bandwidth Memory (HBM) enabled-FPGAs bring tremendous performance potentials. 
Graph processing explores the irregular structure of a graph rather than performing large numbers of computations, resulting in poor data locality and high communication to computation ratio~\cite{graphchallenges,zhu2016gemini}.
As a result, memory bandwidth is the major bottleneck to the system performance. 
Recent FPGAs have started integrating HBM to meet the demand for ever-increasing memory bandwidth of data center applications~\cite{kara2020high,choi2021hbm}. 
For example, Alveo U280~\cite{xilinxu280} equipped with 32 memory channels can deliver up to 460 GB/s of peak memory bandwidth with the given HBM, which is a sixfold increase over the latest FPGA platform equipped with only DRAM memory (Alveo U250~\cite{xilinxu250}). 
This brings great potential in high performance graph processing.


\begin{table}[t!]
\centering
\caption{Estimation of resource utilization of existing designs with increasing the number of memory channels (\#CH). }
\label{table:resource_projection}
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{l|c|rcccc}
\toprule
\begin{tabular}[c]{@{}l@{}}Existing\\ Designs\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Resource\\ Type\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}1 CH\\ (14 GB/s)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}4 CH\\ (58 GB/s)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}8 CH\\ (115 GB/s)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}16 CH\\ (230 GB/s)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}32 CH\\ (460 GB/s)\end{tabular}} \\ \midrule

HitGraph~\cite{zhou2019hitgraph} & LUT  & \cellcolor[rgb]{ .988,  .988,  1} *16.9\% & \cellcolor[rgb]{ .988,  .953,  .965}*68.1\% & \cellcolor[rgb]{ .988,  .906,  .914}136.2\% & \cellcolor[rgb]{ .984,  .808,  .816}272.4\% & \cellcolor[rgb]{ .98,  .612,  .62}544.8\% \\

FabGraph~\cite{ruoshi2019improving}  & LUT &\cellcolor[rgb]{ .988,  .984,  .996} *25.5\% & \cellcolor[rgb]{ .988,  .929,  .941}102.1\% & \cellcolor[rgb]{ .988,  .855,  .867}204.2\% & \cellcolor[rgb]{ .984,  .71,  .718}408.5\% & \cellcolor[rgb]{ .973,  .412,  .42}817.0\% \\

ISCA'21~\cite{isca2021}  & LUT & \cellcolor[rgb]{ .988,  .988,  1} 18.6\% & \cellcolor[rgb]{ .988,  .949,  .961}*74.2\% & \cellcolor[rgb]{ .988,  .894,  .906}148.4\% & \cellcolor[rgb]{ .984,  .788,  .8}296.8\% & \cellcolor[rgb]{ .98,  .576,  .584}593.6\% \\

ThunderGP~\cite{chen2021thundergp}  & CLB  &\cellcolor[rgb]{ .988,  .988,  1} 21.3\% & \cellcolor[rgb]{ .988,  .941,  .953}*85.3\% & \cellcolor[rgb]{ .988,  .878,  .89}170.6\% & \cellcolor[rgb]{ .984,  .757,  .769}341.2\% & \cellcolor[rgb]{ .976,  .51,  .518}682.4\% \\ \bottomrule
\end{tabular}
}
\begin{tablenotes}[flushleft]
\item {*Numbers are obtained from corresponding papers and normalized to U280 while others are proportionally scaled with the number of memory channels.}
\item{*Note the maximal LUT usage in practice is less than 80\%.}
\end{tablenotes}
\end{table}


The extended number of memory channel and capacity of memory bandwidth enable us to create more concurrent graph processing pipelines to utilize the memory bandwidth and improve the system performance,
however, existing designs can not be scaled due to the heavy and monolithic pipeline designs.
Table~\ref{table:resource_projection} presents the estimated resource utilization of existing designs on U280~\cite{xilinxu280}, the largest HBM-enabled FPGA on market, where we obtain the resource usage from corresponding papers and proportionally project them with the number of utilized memory channels. 
It turns out that even when only 8 of the 32 memory channels are used, all designs exceed resource capacity.
Conventional designs tend to build monolithic pipelines that employ extensive techniques to provide high performance for a wide range of graph partitions to provide the efficient data access caused by the inevitable irregular graph structure even after the partitioning~\cite{Zhou2018CF,Zhou2016,ForeGraph,graphgen,zhou2019hitgraph,chen2019fly,chen2021thundergp,isca2021,ruoshi2019improving, graphpartitioning,Chaos,sun2017graphgrind}. 
Such overprovisioned pipeline design result in high resource utilization that prohibits the further scaling of the graph processing system to benefit from the given memory bandwidth.

The monolithic pipeline designs further lead to low resource efficiency when the pipelines process diverse workload of the partitions.
As an instance, partitions with extremely poor locality requires different memory optimization technique and different hardware architecture design that is not necessary for the partitions with good locality, providing equal support to both data access pattern in a single pipeline results in inefficient run-time hardware utilization.


Inspired by the high area efficiency of Heterogeneous Multi-Core Architectures (HMAs)~\cite{kumar2004single,hma,mittal2016survey}, in this paper, we propose lightweight heterogeneous pipeline architectures for resource-efficient graph processing. 
In particular,
\begin{itemize}[leftmargin=*]
    \item We classify graph partitions to two types: dense and sparse partitions by applying a lightweight vertex reordering technique; The dense partitions have the high-degree vertices, with good locality, and the sparse partitions have the low-degree vertices, with low locality. Then we customize two types of pipelines: Little and Big pipelines, to process the different workloads.
    \item We propose a graph-aware task scheduling method that maps partitions to the suitable pipeline types based on the proposed performance model, determines the most efficient pipeline combination, and balances workloads of pipelines.
    \item We develop an automated end-to-end framework--ReGraph, to ease the entire process, which generates efficient deployable graph accelerators with user-defined functions and perform the design sapce exploration in a push-button manner. 
    \item {The comprehensive evaluation shows ReGraph delivers 1.6$\times$--5.9$\times$ performance speedup and 12$\times$ resource efficiency improvement over state-of-the-arts. ReGraph on a budget HBM-enabled FPGA platform provides up to 18$\times$ energy efficiency than GPUs on certain applications.}
\end{itemize}




{The rest of the paper is organized as follows. We motivate our design in Section~\ref{sec:motivation} and introduce system architecture in Section~\ref{sec:systemdesign}.
The performance modeling and task scheduling are presented in Section~\ref{sec:performancemodelingtaskscheduling}.
We present ReGraph framework in Section~\ref{sec:framework}.  
We conduct a comprehensive evaluation in Section~\ref{sec:evaluation}. 
We discuss related work in Section~\ref{sec:relatedwork} and conclude our work in Section~\ref{sec:conclusion}.
}

==> backup.tex <==
\begin{table}[]
\centering
\caption{Resource projection of existing works with increasing number of memory channels.}
\label{table:resource_projection}
\setlength{\tabcolsep}{2.5pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{l|lllll|lllll}
\toprule
Resource Type & \multicolumn{5}{c|}{\textbf{LUT}}  & \multicolumn{5}{c}{\textbf{CLB}} \\ \midrule
\#Mem Channel & \multicolumn{1}{c}{\textbf{1}} & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c|}{\textbf{32}} & \multicolumn{1}{c}{\textbf{1}} & \multicolumn{1}{c}{\textbf{4}}        & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{32}} \\ \midrule
HitGraph~\cite{zhou2019hitgraph}   & 22\%                  & 90\%                  & 181\%                 & 363\%                  & 726\%                   & 22\%                  &90\% & 181\%                 & 363\%                  & 726\%                  \\
FabGraph~\cite{ruoshi2019improving}   & 23\%                  & 93\%                  & 186\%                 & 373\%                  & 747\%                   & 23\%                  & 93\%                         & 186\%                 & 373\%                  & 747\%                  \\
ISCA'21~\cite{isca2021}    & 18\%                  & 75\%                  & 150\%                 & 300\%                  & 600\%                   & 18\%                  & 75\%                         & 150\%                 & 300\%                  & 600\%                  \\
ThunderGP~\cite{chen2021thundergp}  & 21\%                  & 85\%                  & 170\%                 & 340\%                  & 680\%                   & 21\%                  & 85\%                         & 170\%                 & 340\%                  & 680\%                  \\ \bottomrule
\end{tabular}
}
\end{table}


HitGraph~\cite{zhou2019hitgraph} & LUT  & *16.9\% & *68.1\% & 136.2\% & 272.4\% & 544.8\% \\

FabGraph~\cite{ruoshi2019improving}  & LUT & *25.5\% & 102.1\% & 204.2\% & 408.5\% & 817.0\% \\

ISCA'21~\cite{isca2021}  & LUT &  18.6\% & *74.2\% & 148.4\% & 296.8\% & 593.6\% \\

ThunderGP~\cite{chen2021thundergp}  & CLB  & 21.3\% &*85.3\% & 170.6\% & 341.2\% & 682.4\% \\ \bottomrule


HitGraph~\cite{zhou2019hitgraph} & LUT  & \rowcolor[rgb]{ .353,  .541,  .776} *16.9\% & \cellcolor[rgb]{ .796,  .851,  .929}*68.1\% & \cellcolor[rgb]{ .988,  .953,  .965}136.2\% & \cellcolor[rgb]{ .984,  .847,  .855}272.4\% & \cellcolor[rgb]{ .98,  .631,  .639}544.8\% \\

FabGraph~\cite{ruoshi2019improving}  & LUT &\rowcolor[rgb]{ .427,  .592,  .8} *25.5\% & \cellcolor[rgb]{ .988,  .98,  .992}102.1\% & \cellcolor[rgb]{ .988,  .898,  .91}204.2\% & \cellcolor[rgb]{ .984,  .737,  .749}408.5\% & \cellcolor[rgb]{ .973,  .412,  .42}817.0\% \\

ISCA'21~\cite{isca2021}  & LUT & \rowcolor[rgb]{ .365,  .549,  .78} 18.6\% & \cellcolor[rgb]{ .847,  .89,  .949}*74.2\% & \cellcolor[rgb]{ .988,  .945,  .957}148.4\% & \cellcolor[rgb]{ .984,  .827,  .835}296.8\% & \cellcolor[rgb]{ .98,  .592,  .6}593.6\% \\

ThunderGP~\cite{chen2021thundergp}  & CLB  &\rowcolor[rgb]{ .388,  .565,  .788} 21.3\% & \cellcolor[rgb]{ .945,  .957,  .984}*85.3\% & \cellcolor[rgb]{ .988,  .925,  .937}170.6\% & \cellcolor[rgb]{ .984,  .792,  .8}341.2\% & \cellcolor[rgb]{ .976,  .522,  .529}682.4\% \\ \bottomrule



\begin{figure}[htbp]
\begin{tabular}{p{1\linewidth}p{1\linewidth}}
    \begin{minipage}{.5\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{figures/ppb_arch-crop.pdf}
    \caption{Figure one.}
    \label{fig:fig1}
    \end{minipage}
    &
    \begin{minipage}{.5\linewidth}
\begin{lstlisting}
#include <stdio.h>

 main()
 {
    printf ("Hello World!\n");
 }
\end{lstlisting}
\end{minipage}
\end{tabular}
\end{figure}
%\caption{The HLS code snippet of ping-pong buffering.}
%\label{listing:ppb}
%\end{listing}



\begin{figure}[h]
\begin{minipage}{.7\textwidth}  %listing bloc will have 50% of the line width 
\lstset{linewidth = .5\textwidth, breaklines=true} %set your listing lines widths, and set breaklines to true
\begin{lstlisting}[language=C++]
void PPB(&hls::streams){
ap_uint<512> buffer[N][2][SIZE];
w_round = r_round = 0;
while (true){
#pragma HLS PIPELINE II=1
/* logic for writing buffers */
if((w_round - r_round) <= 1){
 for (int u = 0; u < N; u++){
  writ to buffer[u][w_round& 0x1][w_idx];}
  w_idx ++;
 /* early skip */
 if (r_round > w_round){
   w_round = r_round; w_idx = 0;}
 if (w_idx==SIZE){
   w_round ++; w_idx = 0;}}
/* logic for reading buffers */
if(r_round < w_round){
 read_stream(a_src_set);
 r_round = last_src/SIZE;}
if(r_round < w_round){
 for (int u = 0; u < N; u++){ 
  r_idx = src[u] & (SIZE-1);
  read from buffer[u][r_round& 0x1][r_idx];}
  ...
}}
\end{lstlisting}
\end{minipage}
\begin{minipage}{0.2\textwidth} 
%figure will have the remaning 40% of the line width
\includegraphics[width=1\linewidth]{figures/ppb_arch-crop.pdf}  %the image must be resized or scaled if needed
\caption{caption}
\end{minipage}
\end{figure}


\vspace{1mm}
\noindent
\textbf{Streaming Buffer.}
\subsubsection{RAW Solver for URAMs}
The accumulation operation of the Gather PEs potentially introduces read after write (RAW) hazards as the read latency of URAMs is three cycles.
%We simplify the RAW solver of ThunderGP by using shift registers and integrating it into the Gather PEs. 
We hence design an efficient RAW solver with a set of shift registers that buffers the latest updates. 
An incoming update tuple is first compared with the buffered tuples. 
If there is a match, we use the buffered value as one of the operands of the accumulator instead of the value from URAMs (as the value is not the newest one). The updated value will be written to URAMs directly. 
Meanwhile, every buffered tuple in shift registers shifts from the current location to the next location, and the latest update value and destination vertex are appended to the beginning of the registers. 
%Our design avoids complex combination logic introduced in the original design, hence saving a large portion of resources for the RAW solver.

\begin{listing}
\begin{minted}[xleftmargin=14pt,breaklines,linenos,fontsize=\scriptsize,fontfamily=tt,baselinestretch=0.8]{c}
void PPB(...){
ap_uint<512> buffer[ns][2][SIZE];
w_round = r_round = 0;
while (true){
#pragma HLS PIPELINE II=1
/* logic for writing buffers */
if((w_round - r_round) <= 1){
 for (int u = 0; u < N; u++){
  writ to buffer[u][w_round& 0x1][w_idx];}
  w_idx ++;
 /* early skip */
 if (r_round > w_round){
   w_round = r_round; w_idx = 0;}
 if (w_idx==SIZE){
   w_round ++; w_idx = 0;}}
/* logic for reading buffers */
if(r_round < w_round){
 read_stream(a_src_set);
 r_round = last_src/SIZE;}
if(r_round < w_round){
 for (int u = 0; u < N; u++){ 
  r_idx = src[u] & (SIZE-1);
  read from buffer[u][r_round& 0x1][r_idx];}
  ... }}
\end{minted}
\caption{The HLS code snippet.}
\label{listing:ppb}
\end{listing}

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.4\linewidth]{figures/ppb_arch-crop.pdf}
  \label{fig:ppb}
  \caption{The architecture and data flow of ping-pong buffering, assuming the Big pipeline process four edges per cycle. Orange lines indicate fetched vertex property.}
\end{figure}



\begin{table}
\centering
\caption{The graph applications.}
\label{table:graphapplication}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{ll}
\toprule
\multicolumn{1}{l}{Apps}   & Description \\ 
\midrule
\multicolumn{1}{l|}{PR}  & Scores the importance and authority of a website through its links\\ 
\multicolumn{1}{l|}{SpMV}  & Multiplies a sparse matrix (represented as a graph) with a vector\\ 
\multicolumn{1}{l|}{BFS}   & Traverses a graph in a breadth ward from the selected node \\ 
\multicolumn{1}{l|}{SSSP}  & Finds the shortest path from a selected node to another node\\ 
\multicolumn{1}{l|}{CC}  & Detects nodes which could spread information very efficiently\\ 
\multicolumn{1}{l|}{AR}  &  Measures the transitive influence or connectivity of nodes\\ 
\multicolumn{1}{l|}{WCC}  & Finds maximal subset of vertices with weak connection\\ 
\multicolumn{1}{l|}{SCC}  & Finds maximal subset of vertices with strong connection\\ 
\bottomrule
\end{tabular}
}
\end{table}


% \begin{table}[]
% \begin{tabular}{@{}|l|l|l|l|l|@{}}
% \toprule
% Pipeline Type   & \multicolumn{1}{c|}{Vertex Access} & \multicolumn{1}{c|}{Update dispatching} & Target Partition  & \multicolumn{1}{c|}{Features} \\ \midrule
% Big Pipeline    & Streaming Buffer                   & Data Routing                            & Sparse Partitions & Poor Locality; Small Workload \\ \midrule
% Little Pipeline & PingPing Buffering                 & Static dispatch                         & Dense Partitions  & Good Locality; Large Workload \\ \bottomrule
% \end{tabular}
% \end{table}



\begin{figure}[h!]
  \centering
  \includegraphics[width=1\linewidth]{figures/ligra_pr-crop.pdf}
  \caption{ReGraph compared to Ligra on PR.}
  \label{fig:ligra_pr}
\end{figure}
\begin{figure}[h!]
  \centering
  \includegraphics[width=1\linewidth]{figures/ligra_bfs-crop.pdf}
  \caption{ReGraph compared to Ligra on BFS.}
  \label{fig:ligra_bfs}
\end{figure}


\begin{figure}[h!]
\centering
\begin{subfigure}[t]{.17\textwidth}
  \includegraphics[width=1\linewidth]{figures/gunrock_pr-crop.pdf}
  \caption{PR.}
  \label{fig:gunrock_pr}
\end{subfigure}%
\hspace{0.1mm}
\begin{subfigure}[t]{.156\textwidth}
  \includegraphics[width=1\linewidth]{figures/gunrock_bfs-crop.pdf}
  \caption{BFS.}
  \label{fig:gunrock_bfs}
\end{subfigure}%
\hspace{0.1mm}
\begin{subfigure}[t]{.147\textwidth}
  \includegraphics[width=1\linewidth]{figures/gunrock_cc-crop.pdf}
  \caption{CC.}
  \label{fig:gunrock_cc}
\end{subfigure}%
\caption{ReGraph compared to Gunrock on Tesla P100.}
\label{fig:gunrockcompare}
\end{figure}


\subsection{Impact of Task Scheduling}\label{sec:benefitsof}
We study the impact of key parameters in task scheduling, including the numbers of Little and Big pipelines $(M, N)$ and the numbers of dense and sparse partitions $(X, Y)$. 
%We enumerate every possible configuration to find the best performance. In other words, we run graphs in
%We vary the numbers of Little and Big pipelines from (0, 14) to (14, 0) and the number of dense partitions until the performance trends are converged. In other words, we mark the first to the $X$ partitions as dense partitions and the rest $Y$ partitions as sparse ones. 
To find the best configurations, we run graphs on all possible pipeline combinations and vary the number of dense partitions.
{Table~\ref{table:systemperformance} shows the performance of three applications with the best parameters and the inter-cluster scheduling method selected parameters.}
Figure~\ref{fig:bestconfigurations} depicts the best parameters of PR on U280. We only present the numbers of dense partitions and Little pipelines, as the rest of the partitions are sparse and the rest of the pipelines are Big pipelines. 
%other two parameters can be calculated according to the total numbers of partitions and pipelines. 
%where the size of the marker indicates the times the configuration has been selected. 

There are several highlights.
Firstly, the peak performance is up to 19,028 MTEPS (CC with HW). 
Secondly, the geometric mean of our system selected parameters can approach 91\%, 92\%, and 91\% of that of the best parameters on three applications.
Thirdly, from Figure~\ref{fig:bestconfigurations}, the best configurations are with mixed pipeline types rather than a single type, indicating the benefits of heterogeneity. 
They roughly have similar numbers of Big and Little pipelines, suggesting both types of pipelines play an equally important role in performance.
Fourthly, synthetic graphs (R19, R21, R24 and G23) have better performance and require more Little pipelines than real-world graphs, because they are relatively regular and have larger portion of edges located in dense partitions. 
%Lastly, large graphs usually have more dense partitions. 


% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=1\linewidth]{figures/Scalibility-crop.pdf}
%   \caption{Performance of PR with varying the number of utilized memory channels on U280.}
%   \label{fig:scalibility}
% \end{figure}


\begin{table*}[h!]
\centering
\caption{The performance (MTEPS) of three applications with best parameters (Best) and the parameters selected by the proposed task scheduling model (System) on U280.}
\label{table:systemperformance}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l|c|llllllllllllllll|c|c@{}}
\toprule
\multicolumn{1}{c|}{APPs}                                   & Config & \multicolumn{1}{c}{R19} & \multicolumn{1}{c}{R21} & R24  & \multicolumn{1}{c}{G23} & GG    & AM   & HD     & BB    & TC   & PK  & FU  & WP  & LJ  & HW   & DB   & OR  & Geo Mean & \multicolumn{1}{c}{Acc.} \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{PR}} & Best  & 13169                   & 15253                   & 9915 & 13764                   & 4946 & 4224 & 7662 & 7286 & 7920 & 8087 & 9530 & 7658 & 8853 & 15420 & 5457 & 12364 & 8834 & \multicolumn{1}{c}{\multirow{2}{*}{91\%}}         \\
\multicolumn{1}{c|}{}                    & System  &12525	&13340	&9815	&13179	&3782	&3744	&6939	&6875	&7790	&7442	&8948	&7659	&6414	&13768	&5230	&11315	&8037 &                            \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{{BFS}}}                    & Best  & 12661 & 13772 & 9554  & 12974 & 4595  & 4060   & 6877  & 6754  & 7495  & 7378  & 8861 & 7086  & 6336  & 14967 & 5229  & 12158 & 8167
 & \multicolumn{1}{c}{\multirow{2}{*}{92\%}}        \\
                                         & System  &9951	&13011	&9421	&12712	&3397	&4060	&5854	&6161	&7089	&7006	&10350	&7086	&5934	&13773	&4263	&11279	&7545  &                           \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{{CC}}}                     & Best  & 12992 & 17279 & 10718 & 14273 & 5087  & 4583  & 7672  & 7375 & 8574  & 7993  & 9858  & 7816  & 7024  & 19028 & 5939  & 14588 & 9229
 & \multicolumn{1}{c}{\multirow{2}{*}{91\%}}         \\
                                         & System  &12570	&17227	&10718	&14273	&4065	&4152	&6529	&7375	&7640	&7680	&7712	&7816	&6426	&16926	&5130	&10602	&8354 &                              \\ \bottomrule
\end{tabular}
}
\end{table*}


% \subsection{Impact of DBG Reordering}\label{sec:vertexreorderingimpact}
% %We evaluate the efficacy of degree-based grouping with different granularities~\cite{DBG}.
% Figure~\ref{fig:dbg} shows the performance of PR with different grouping granularities of DBG. 
% Preprocessing without vertex grouping is used as the baseline. 
% In the figure, `DBG(8)' means vertices are grouped into eight groups based on eight in-degree ranges. `Sorting' is the extreme case of DBG with as many number of groups as many unique degrees a given dataset has.
% %where vertices are sorted based on their in-degrees. 
% %`Sorting' can be seen as an implementation of DBG algorithm with as many number of groups as many unique degrees a given dataset has. 
% Clearly, DBG and sorting can significantly improve performance compared to the baseline, as they make the heterogeneity of partition workloads more extreme, with the first few partitions super dense and others super sparse. DBG(16) and DBG(32) outperform sorting slightly, as sorting leads to edges within partitions unbalanced. 
% In general, grouping vertices into 16 groups is a suitable granularity for high performance on all evaluated graphs.


% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=1\linewidth]{figures/dbg-crop.pdf}
%   \caption{PR Performance with varying DBG settings on U280.}
%   \label{fig:dbg}
%   \vspace{-3mm}
% \end{figure}

\vspace{0.5mm}\noindent
\textbf{HLS optimizations.}
HLS partially solves the programmability issue of FPGAs. Efficient HLS designs still require hardware knowledge and significant development efforts.  
A number of works have been proposed to improve the efficiency of HLS implementations~\cite{HLSsurvey,chen2018architectural,wang2016performance,Li2017,cong2017bandwidth,cong2018automated,Shuo2017,workstealing,ST-Accel}. 
%In particular, Cong et al.~\cite{cong2018automated} proposed a composable architecture template to reduce the design space of HLS designs. They also presented buffer restructuring approaches to optimize the bandwidth utilization with HLS ~\cite{cong2017bandwidth}.  
%Wang et al.~\cite{wang2016performance} proposed an analytical framework for tuning the pragmas of HLS designs. 
In this paper, we provide highly optimized accelerator templates, platform-specific optimizations and even code generation for users so as to ease the development process. 

\vspace{0.5mm}\noindent
\textbf{HBM exploration.}
The research community has been actively exploring how best to use the many channels of HBM. 
Yang et al.~\cite{yang2020high} proposed a high throughput parallel hash table accelerator on HBM-enabled FPGAs.
{Liu et al. proposed ScalaBFS~\cite{liu2021scalabfs} that also uses multiple PEs to exploit the high bandwidth of HBM for BFS.}
Kara et al.~\cite{kara2020high} implemented three data analytic workloads by duplicating pipelines to demonstrate benefits of HBM. 
Since any congestion on a particular memory channel reduces the effective bandwidth when utilizing the built-in crossbar, they use HBM channels independently. {Similarly, Choi et al.~\cite{choi2021hbm} argued the potential bandwidth bottleneck from the shared links of the built-in crossbar. ReGraph also uses HBM channels independently.
%, but instead of homogeneous pipelines or PEs, we propose heterogeneous pipeline architectures for scaling the number of pipelines.
}


\vspace{1mm}
\noindent
\textbf{Data Router.}
Data router dynamically dispatches update tuples to Gather PEs that buffer their destination vertices.
%; hence, buffers of gather PEs could accommodate distinctive vertices, enlarging the partition size. 
{Although Chen et al. proposed an efficient OpenCL-based data shuffling solution~\cite{chen2019fly}, it remains resource intensive due to the large number of replicas of tables for decoding.}
We propose a lightweight dataflow-based architecture, which steers data through a multi-layer merge tree to amortize overhead caused by potential conflicts~\cite{chen2019fly}. 

Figure~\ref{fig:datarouting} illustrates the data flow of the Data Router, assuming four update tuples are dispatched to four Gather PEs.
In the first stage, four Dispatchers read four update tuples (with the format of $\langle value, dst \rangle$) in parallel and assign tuples to local streams based on destination PE IDs (calculated by $ dst \mod 4 $). 
%As Dispatchers are processing independently, they can process four tuples per cycle. 
A two-level merge-tree is then used to merge tuples with same destination PE IDs to one stream.
The first level contains eight $2\times1$ Mergers, and each of them merges two streams with the same ID from two Dispatchers into one local stream. 
Similarly, in the second level, four $2\times1$ Mergers merge eight streams to four streams that are directly connected to Gather PEs.
The proposed architecture follows the dataflow execution model and is fully pipelined with HLS. 


\begin{figure}[t!]
\begin{subfigure}{.5\linewidth}\centering  %listing bloc will have 50% of the line width 
\lstset{linewidth = \textwidth, basicstyle=\scriptsize\ttfamily, breaklines=true} 
\begin{lstlisting}[language=C++]
void PPB(...){
ap_uint<512> buf[2][nspe];
wid = rid = 0;
while(true){
#pragma HLS PIPELINE II=1
// logic for filling buffers
if((wid - rid) <= 1){
 write to buf[wid&1];}
if(buf is full){
  wid ++; 
  reset buf pointer;}}
if(rid > wid){
  wid = rid; // jump access
  reset buf pointer;}
// logic for reading buffers
if(rid < wid){
 read one src set;
 rid = last_src/SIZE;}
if(rid < wid){
  read from buf[rid&1];}
  ...
}}
\end{lstlisting}
\vspace{-6mm}
\caption{HLS code snippet.}
\label{fig:ppbhls}
\end{subfigure}
\begin{subfigure}{0.45\linewidth}\centering
\includegraphics[width=\textwidth]{figures/ppb_arch-crop.pdf} 
\caption{Micro-architecture.}
\label{fig:ppbarch}
%the image must be resized or scaled if needed
\end{subfigure}
\caption{The HLS code snippet and micro-architecture of the Ping-Pong Buffer.}
\label{fig:ppb}
\end{figure}


  \begin{figure}[h!]
     \centering
    \begin{minipage}[b]{1\linewidth}
     \includegraphics[width=1\linewidth]{figures/ligra_pr-crop.pdf}
    \caption{ReGraph compared to Ligra on PR.}
    \label{fig:ligra_pr}
    \end{minipage}

    \begin{minipage}[b]{1\linewidth}
    \includegraphics[width=1\linewidth]{figures/ligra_bfs-crop.pdf}
    \caption{ReGraph compared to Ligra on BFS.}
    \label{fig:ligra_bfs}
    \end{minipage}
    
    \begin{minipage}[b]{1\linewidth}
    \begin{subfigure}[t]{.352\textwidth}
      \includegraphics[width=1\linewidth]{figures/gunrock_pr-crop.pdf}
      \caption{PR}
      \label{fig:gunrock_pr}
    \end{subfigure}%
    \hspace{0.1mm}
    \begin{subfigure}[t]{.32\textwidth}
      \includegraphics[width=1\linewidth]{figures/gunrock_bfs-crop.pdf}
      \caption{BFS}
      \label{fig:gunrock_bfs}
    \end{subfigure}%
    \hspace{0.1mm}
    \begin{subfigure}[t]{.302\textwidth}
      \includegraphics[width=1\linewidth]{figures/gunrock_cc-crop.pdf}
      \caption{CC}
      \label{fig:gunrock_cc}
    \end{subfigure}%
    \caption{ReGraph compared to Gunrock on Tesla P100.}
    \label{fig:gunrockcompare}
    \end{minipage}
  \end{figure}

